Internet Congestion Control via Deep Reinforcement Learning

We present and investigate a novel and timely application domain for deep reinforcement learning (RL): Internet congestion control. Congestion control is the core networking task of modulating traffic sources' data-transmission rates to efficiently utilize network capacity, and is the subject of extensive attention in light of the advent of Internet services such as live video, virtual reality, Internet-of-Things, and more. We show that casting congestion control as RL enables training deep network policies that capture intricate patterns in data traffic and network conditions, and leverage this to outperform the state-of-the-art. We also highlight significant challenges facing real-world adoption of RL-based congestion control, including fairness, safety, and generalization, which are not trivial to address within conventional RL formalism. To facilitate further research and reproducibility of our results, we present a test suite for RL-guided congestion control based on the OpenAI Gym interface.

==> cc.tex <==
\section{Challenges}

\NR{Why is this problem interesting from an ML point of view?}

\subsection{Enormous Search Space}
Each actions is the sender's new rate, which, being a real number, has infinite possibilities.
\AT{Actually, this is a scalar action, and we expect some continuity in it, so I wouldn't claim this as being enormous (standard tasks in Gym have tens of continuous dimensions)}

\subsection{Continuous State}
Our state is made of statistics vectors, comprised of sending and receive rates, corresponding reward, as well as properties of the environment as viewed by the sender (loss rate and latency)
\NJ{Is continuous state a serious problem, given the availability of policy graident methods?}

\subsection{Dynamic Environment}


% \subsection{Complex, Dynamic Environment}
% The environment in which Internet congestion control operates can contain many moving parts. 
% First, the number of senders and receivers can change at any given time. The congestion control algorithm each sender employs can vary greatly, from ones of a "greedy" nature, to whose who wish to utilize only the resources that are available ("scavenger").




\subsection{Evaluation of States and Effects of Actions is Hard}
\NJ{That may be true with many senders, but I'm not sure it's true for us.}

\subsection{Performance Measurement}
The Internet today has many uses. As such, each sender may have different and at times conflicting goals. Some applications, such as Voice over IP (VoiP,~\cite{x}), may require packets to arrive very quickly in order to function effectively. These application strive to reduce the amount of time it takes a packet to traverse through a network, termed \textit{latency}.
Another fundamental measurement of network quality is \textit{throughput} - the rate in which packets arrive successfully at the receiver. Increasing throughput is the goal of very popular applications such as file downloads.

Traditional approaches to congestion control take into account another form of quality measurement: loss rate, and uses it as an indication of congestion. This is not a sound policy, as other factors, related to the physical component of the network,  contribute to its loss rate~\cite{bbr}.

The relation between latency, throughput and loss rate is therefore quite intricate, involving many varying elements. 
\NR{add more here?}.
As application requirements differ, the networking community adapted the approach of considering both increased throughput and reduced latency as a performance measure.
% As one application might prefer one of these measures the other, the performance measurement accepted by the community is increasing throughput while reducing latency simultaneously.



\subsection{Effect of event horizon}
\NR{Right now, \autoref{fig:discount_factor} shows that gamma isn't really a factor. To some reviewers, this might indicate that this is not really an RL problem. We need a discussion here - maybe in some scenarios, i.e.  smaller buffers / BW this isn't the case?}
\AT{Can we generate a toy domain where discount factor would be important? Then, we can say that in theory it should, so perhaps better RL algorithms would eventually make use of it, but for now our results show that it's not a significant component in the decision making.}
\NJ{Just to help discussion, I've added the figure for training with three different values of gamma below. It does appear to matter.}\AT{This is quite a weird result. Are you sure about it? Almost always, reducing the discount factor leads to more stable training. Here it seems that for the lower discount factors the training is very unstable.}

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/cc_gamma_reward_graph.png}
    \caption{Training reward for models with three different discount factors. Three replicas of each model are trained, with the average training reward smoothed and plotted. Models with a low discount factor appear to improve barely, if at all for the same number of episodes that produces a reasonble model using a discount factor of 0.99.}
    \label{fig:intro_random_loss}
\end{figure}

\subsection{Fairness}

The users sending data over the Internet may use very different congestion control algorithms. Instead of trying to train our agent to compete or cooperate with other senders, a situation that can only be achieved by simulation and is not similar to the real-world settings, in chapter *** we discuss the results our RL agent achieves for multipflow scenarios.
% We did not train our agent in environments where it competed or cooperated with another sender.

% In all its training, our agent neither competed nor cooperated with another sender, so we had little expectation for its multiflow performance. 
% Figure \autoref{fig:fairness} shows Jain's Fairness Index computed for a set of competing senders with various numbers of competitors for several congestion control schemes. With just two senders, our agent is extremely unfair, with one sender taking a greater and greater share of the bandwidth after the two senders initially diverge by only a small amount. With more senders though, our agent is actually more fair. We suspect this is due in large part to randomness in the timing of the senders. With just two senders, the one that loses bandwidth always gives it to the same opponent. With four senders, the extra bandwidth might be given away randomly or distributed among competitors, preventing one flow from dominating as significantly. Improving our agent's robustness to multiflow competition is an interesting avenue for future work, a point of discussion in 


% As our evaluation shows \NR{need to add those results}, our agent was reasonably fair when competing with itself, despite our every suspicion that it wouldn't be (we used neither global optimization as in Remy~\cite{remy}, nor game-theory-guided utility functions as in~\cite{allegro, vivace}). Despite this, our agent may not be friendly to TCP. Worse yet, if it were trained in an environment where it selfishly competed with TCP, it might occasionally induce packet loss just to force TCP into backing off. Can our RL agent be trained to ``play well'' with other protocols (TCP, PCC~\cite{allegro,vivace}, BBR~\cite{bbr}, Copa~\cite{copa})?

Can the RL agent learn to interact with another agent fairly? Can it be fair to TCP? If it could be trained not to compete with TCP, could an agent detect bandwidth that is unused by TCP and use only that?

Beyond straightforward competition with TCP, an RL agent might learn interesting methods of cooperation or deception. BBR~\cite{bbr} and Copa~\cite{copa} both use coordinated buffer draining phases to obtain a measure of base RTT and build a model of available bandwidth. A cooperative RL agent might back off at the same time to help the other flows perform well, while a competitive one may ramp up, or cause latency oscillations that prevent BBR or Copa from constructing sensible network models. 

\AT{Generalization should appear here in the discussion.}

\AT{Another issue can be safety: can we know when the network is uncertain about its action, and in this case fall back to some baseline policy?}

==> discussion.tex <==

\section{Discussion and Future Research}
% \label{sec:discussion}

Our work so far has provided a foundation for reinforcement learning in congestion control, but leaves open a variety of interesting research questions.

\sub{How can we make RL agents interact with other flows optimally?}
As our evaluation shows, our agent was reasonably fair when competing with itself, despite our every suspicion that it wouldn't be (we used neither global optimization as in Remy~\cite{remy}, nor game-theory-guided utility functions as in~\cite{allegro, vivace}). Despite this, our agent may not be friendly to TCP. Worse yet, if it were trained in an environment where it selfishly competed with TCP, it might occasionally induce packet loss just to force TCP into backing off. Can our RL agent be trained to ``play well'' with other protocols (TCP, PCC~\cite{allegro,vivace}, BBR~\cite{bbr}, Copa~\cite{copa})?

%If it could be trained not to compete with TCP, could an agent detect bandwidth that is unused by TCP and use only that?

%Beyond straightforward competition with TCP, an RL agent might learn interesting methods of cooperation or deception. BBR~\cite{bbr} and Copa~\cite{copa} both use coordinated buffer draining phases to obtain a measure of base RTT and build a model of available bandwidth. A cooperative RL agent might back off at the same time to help the other flows perform well, while a competitive one may ramp up, or cause latency oscillations that prevent BBR or Copa from constructing sensible network models. 

\sub{Is this method of congestion control practical?}
Many congestion control algorithms have very low overhead. With calls to the sluggish python interface for tensorflow, our model takes about 100us to make a rate decision. Thankfully, work on learned hash functions suggests that small neural networks can be made extremely fast \cite{learned_hashing}. 

%The lack of guaranteed behavior may be more fundamentally upsetting than the speed. Simply providing rate bounds limits the technology we can use, and it has two orders of magnitude range (say 1 to 100mbps), then it's still possible for our agent to choose a rate with either 1\% throughput, or 99\% loss rate, depending on the link capacity. Bounds based on network conditions may be somewhat more sensible. The model could be prevented from sending data when the observed loss rate is above 10\% loss rate, or when the latency is more than double the base latency of a connection. These limits require assumptions about network conditions though, and where they are violated, performance will suffer. The best performing agent will probably be well trained but unconstrained.

\sub{What other inputs can we use to improve our models?} We imagine that real world deployments might include inputs like time of day to learn about diurnal congestion patterns, IP address information to learn about likely network technologies, port information to learn about application traffic patterns, or geographical information to learn about expected latency and capacity. We leave this to future work. 
% \AT{want to mention meta learning~\cite{finn2017model} for quickly adapting to changes in the traffic?}

%\sub{Who should be training their own agents?}
%Operators of large networks might already write their own variants on TCP, or even their own complete congestion control algorithms (as with BBR \cite{bbr} at Google). We expect such communities would be interested in training specialized models for their network, perhaps not just one model per objective, but different models for each datacenter's outbound traffic, or point of presence. We envision a much wider audience though. Our training required only a few hours on four CPU cores, so it is accessible to anyone with a modern computer. It might be reasonable for every desktop, or even every device to have a specialized congestion control agent that learns over time to deal with the oddities of a particular configuration or usage pattern.

\sub{Can we leverage ML even further?}
%While our work certainly enjoys the benefit of ML, we want to push the envelope even further. 
As mentioned in \autoref{subsec:design_architecture}, when it comes to the architecture of the neural network, we have barely scratched the surface. In addition, we wish to explore in future work different RL algorithms, such as~\cite{ppo, a3c}.
% An approach different from ours would be training a different model for each particular set of expected behaviors. This way, a model may be better tailored to specific network environments. As each scenario may present different challenges, and therefore should be explored thoroughly, we plan to delve into this issue in future work
Finally, integrating state-of-the-art ML techniques such as \textit{meta learning}~\cite{finn2017model}, which can be used in conjunction with RL, might help the agent to adapt more swiftly to changes.
% is being used recently on RL frameworks~\cite{x,y}. This additional tool may help our model to better adjust to swift changes such as bursts.


==> motivation.tex <==
\section{Motivation for RL-Guided Rate Control}
\label{sec:motivation}

\NR{Show how RL captures some patterns regular TCP (CUBIC) doesn't.}
\NJ{My understanding of the goal of this section: 1. Show that existing congestion control is not perfect. 2. Discuss why we think reinforcement learning might be better. I'll try to write accordingly. Feel free to put other goals, or help correct me.}

While a traffic source can compute some meaningful network statistics using acknowledgements from the traffic receiver, how these statistics can be used to inform data transmission rates has long been a subject of research. One reason for continued research is an inherent trade off between desirable high link utilization with undesirable congestion (in the form of either latency or packet loss). In many simple network models (i.e. an M/M/1 queue), this trade off \emph{should} be very small. For a single link, a traffic source that can measure the length of the queue can trivially limit the latency while obtaining near-capacity throughput. Unfortunately, networks can be noisy, rapidly-changing and filled with other traffic sources that take independent actions with independent goals.

\NR{Aviv, can you take a look a this paragraph below? I think in this part we should only compare to one BASIC algorithm, i.e. CUBIC, and leave the rest for later, in order to build up the paper more clearly. Thoughts?}\AT{I agree, this section should be as simple and clear as possible.}

In this section, we examine three different network scenarios to demonstrate the challenges and trade offs of existing algorithms. We present results for five algorithms, TCP-Cubic~\cite{ha2008cubic} and BBR~\cite{bbr} (two algorithms commonly used in the real world), Copa~\cite{copa} and PCC-Vivace~\cite{vivace} (two algorithms presented at the most recent iteration of NSDI, a top networking conference), and RemyCC~\cite{remy} (a policy that uses rate control similar to TCP-Cubic, but with rules generated via machine learning). We run each test for 30 seconds using the Pantheon framework to manage traffic sources and receivers~\cite{pantheon}.



\subsection{Basics}
\NR{Showing the Pareto frontier of our RL problem contains the performance of CUBIC for a very basic scenario}
\NJ{I think just a stable link might work for this.}
\NR{Yeah, me too.}

\NR{I think we should introduce the performance measurement here, I don't believe we do it clearly before, and it's needed here.}

Our first example is a single link with a single traffic source. The link is configured with a capacity of 30mbps, a latency of 32ms, 0\% random loss and a maximum queue size of 500 packets. These numbers roughly align with a regional connection using home internet in the U.S. (actual numbers vary widely). In figure XX, we plot the trade off of average throughput and average latency for ten runs of our example congestion control protocols.

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/motivation_stable_tradeoff.png}
    \caption{Congestion control protocols make different trade offs in throughput and latency, but latency-sensitive protocols sacrifice nearly 20\% throughput to keep latency low.
    \NJ{Figure not final, will add the RemyCC algorithm, change background color to white and change scheme names. Feel free to add other suggestions.}}
    \label{fig:motivation_random_loss}
\end{figure}




\subsection{Detecting Random Loss}

\NJ{I have an idea about how to show this. First, we test the schemes with increasing random loss and determine the maximum loss they can tolerate and still maintain 75\% throughput, or something like that. Then, we test multiple copies of the scheme and see what the congestion loss rate is for some number like 8 or 16 copies.}

Packet loss in a network can be the result of real congestion, or be due to hardware random loss along various links. 
Even in the case of real congestion, unless the congestion is caused by the sender, its' sending rate should not decreased (for example, in the case of competing senders).

One of the problems TCP CUBIC is known for is its' innate inability to distinguish between packet loss which is random, congestion not caused by the sender, and congestion indicating that the sender should adapt its' sending rate.

\autoref{fig:motivation_random_loss} demonstrates the behavior of TCP CUBIC pitted against our trained deep RL agent. In this scenario there is a single sender, which is the cause of congestion when it occurs. We tested using different random loss values. Our agent was able to successfully ignore the random loss, increasing the sending rate and gets within *** of the optimal rate. TCP CUBIC, on the other hand, interprets the random packet loss as congestion even when it is sending well below the optimal sending rate, thus decreasing its' sending rate, causing poor performance.

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/random_loss.png}
    \caption{Differentiating between random and non-random loss is a task TCP CUBIC struggles with. Our RL model, on the other hand, trained on three random loss rates, is able to overcome this problem, and generalize to a variety of values.
    \NR{Tmp figure!}}
    \label{fig:motivation_random_loss}
\end{figure}

\subsection{Capturing Patterns in a Dynamic Environment}

\NJ{Multiple schemes, including our own record-keeping relies on a fairly stable base RTT. This is a sensible assumption for the Internet, but it limits what we can change a little bit. Should be able to replicate the Custard experiment here, possibly run an LTE scenario as well.}

Internet congestion control is a highly dynamic environment, with senders joining and leaving, hardware failing, causing changes, sometimes drastic, to the available bandwidth. These conditions require the sender to detect and adapt quickly to change.

We simulated a dynamic environment by changing the bandwidth every five seconds.
\NR{Fill out once we have a better experiment running (smaller buffers so that TCP would go crazy).}
% Here, TCP CUBIC increases its' sending rate rapidly at the beginning of the run, filling the buffer on the sender's end. When the bandwidth suddenly drops, the sender can't send that amount of information so fast, thus increasing the latency.
Our RL agent, on the other hand, learns to react to other subtle signals, namely changes in latency, and do so in proportion to the change in the signal. As shown in \autoref{fig:motivation_jitter}, when there is a spike in latency, the RL agent reacts immediately by dropping its' sending rate. Note that the change in sending rate is in proportionate to the latency spike. Thus, our RL agent is able to maintain both high throughput and low latency.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/jitter_changed.png}
    \caption{Our RL agent, even though it was trained on static environments, manages to learn how to react properly to very dynamic environments. CUBIC, the common solution, does not manage to get low latency - it keeps the sending rate as high as it possibly can, without draining the buffers, causing the latency to remain high at all time. \NR{tmp figure}}
    \label{fig:motivation_jitter}
\end{figure}
